A Reverse Engineering Education Needs Analysis Survey

This paper presents the results of a needs analysis survey for Reverse Engineering (RE). The need for reverse engineers in digital forensics, continues to grow as malware analysis becomes more complicated. The survey was created to investigate tools used in the cybersecurity industry, the methods for teaching RE and educational resources related to RE. Ninety-three (n=93) people responded to our 58 question survey. Participants did not respond to all survey questions as they were optional. The data showed that the majority of 24/71 (33.8%) responses either strongly agreed and 22/71 (30.99%) of responses somewhat agreed that there is a shortage in RE resources. Furthermore, a majority of 17/72 (23.61%) responses indicated that they strongly disagree and that 27/72 (37.5%) somewhat disagree to the statement that graduates are leaving college with adequate RE knowledge. When asked if there is a shortage of adequate RE candidates, the majority of 33/71 (46.48%) responses strongly agreed and 20/71 (28.17%) somewhat agreed. In order to determine if this was a result of the tools at their disposal, a series of questions in regards to the two most popular RE tools were also asked.

==> sections/testtable.tex <==
\begin{table*}[!hbtp]
\begin{center}
\caption*{Table D.1. Free or commercial edition of IDA.}
\begin{tabular}{p{.64\NetTableWidth} p{.12\NetTableWidth} p{.24\NetTableWidth}}
\hline
 \textbf{IDA Edition} & \textbf{Count} & \textbf{Percentage} \\ \hline
Free	    & 25 & 50\% \\
Commercial	& 25 & 50\%	\\\hline
 \end{tabular}
\end{center}
%\end{table}
\label{table:d1}

 
%\begin{table}[!ht]
\begin{center}
\caption*{Table D.2. IDA/IDA Pro GUI features that should be improved.}
\begin{tabular}{p{.64\NetTableWidth} p{.12\NetTableWidth} p{.24\NetTableWidth}}
\hline
 \textbf{Feature} & \textbf{Count} & \textbf{Percentage} \\ \hline 
Debugger	                            & 18 & 30\%	\\
Third-party plugins	                    & 11 & 18.33\%	\\  
Disassembler	                        & 9 & 15\%	\\
Graph view	                            & 6 & 10\% \\
Function call graph	                    & 4 & 6.67\% \\	
Library function signature recognition	& 4 & 6.67\% \\		
Reference table	                        & 3 & 5\% \\
Hex view	                            & 2 & 3.33\% \\	
Variable renaming	                    & 0 & 0.00\% \\
Function signature modification	        & 0 & 0.00\% \\	
Other	                                & 3 & 5\% \\	\hline
 \end{tabular}
\end{center}
\vspace{-0.1in}
%\end{table}
\label{table:d2}

%\begin{table}[!ht]
\begin{center}
\caption*{Table D.3. Does IDA/IDA Pro have any features that are advantageous over those in Ghidra?}
\begin{tabular}{p{.64\NetTableWidth} p{.12\NetTableWidth} p{.24\NetTableWidth}}
\hline
 \textbf{} & \textbf{Count} & \textbf{Percentage} \\ \hline
Yes	& 13 & 48.15\%	\\ 
No	& 14 & 51.85\%	\\ \hline

 \end{tabular}
\end{center}
\vspace{-0.1in}
%\end{table}
\label{table:d3}

%\begin{table}[!ht]
\caption*{Table D.4. Ghidra GUI features that should be improved.}
\begin{center}
\begin{tabular}{p{.64\NetTableWidth} p{.12\NetTableWidth} p{.24\NetTableWidth}}
\hline
 \textbf{Feature} & \textbf{Count} & \textbf{Percentage} \\ \hline
Debugger	                            & 9 & 20.93\%	\\
Graph view	                            & 8 & 18.60\% \\	
Library function signature recognition	& 8 & 18.60\% \\
Function call graph	                    & 6 & 13.95\% \\	
Hex view	                            & 6 & 13.95\% \\	
Disassembler	                        & 3 & 6.98\%	\\  
Function signature modification	        & 1 & 2.33\% \\
Third-party plugins	                    & 1 & 2.33\%	\\	
Data type viewer                        & 1 & 2.33\% \\
Reference table	                        & 0 & 0.00\% \\	\hline
 \end{tabular}
\end{center}
\vspace{-0.1in}
%\end{table}
\label{table:d4}

%\begin{table}[!ht]
\begin{center}
\caption*{Table D.5. Does Ghidra have any features which are better than those in IDA/IDA Pro?}
\begin{tabular}{p{.64\NetTableWidth} p{.12\NetTableWidth} p{.24\NetTableWidth}}
\hline
 \textbf{} & \textbf{Count} & \textbf{Percentage} \\ \hline
Yes	& 13 & 52.00\%	\\ 
No	& 12 & 48.00\%	\\ \hline
 \end{tabular}
\end{center}
\end{table*}
\label{table:d5}
